Inner Monologue: Embodied Reasoning through Planning with Language Models

Recent works have shown how the reasoning capabilities of Large Language Models (LLMs) can be applied to domains beyond natural language processing, such as planning and interaction for robots. These embodied problems require an agent to understand many semantic aspects of the world: the repertoire of skills available, how these skills influence the world, and how changes to the world map back to the language. LLMs planning in embodied environments need to consider not just what skills to do, but also how and when to do them - answers that change over time in response to the agent's own choices. In this work, we investigate to what extent LLMs used in such embodied contexts can reason over sources of feedback provided through natural language, without any additional training. We propose that by leveraging environment feedback, LLMs are able to form an inner monologue that allows them to more richly process and plan in robotic control scenarios. We investigate a variety of sources of feedback, such as success detection, scene description, and human interaction. We find that closed-loop language feedback significantly improves high-level instruction completion on three domains, including simulated and real table top rearrangement tasks and long-horizon mobile manipulation tasks in a kitchen environment in the real world.

==> Closed Loop LLM Planning CoRL 2022 2/extra/implementation_details.tex <==
% \subsection{Figures Moved to Appendix from Main Text}

% % This was moved from main text to save space.
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=1.0\textwidth]{figures/flowchart_decision_making}
%   \caption{\small\textbf{\algname Reacts to Feedback} The planner is able to react to textual feedback from success detector, object detection and human preference. After each environment feedback, the planner updates its predictions in language space for the next action.}
%   \todo{caption}
%   \label{fig:saycan-flow-chart}
% \end{figure}

% \begin{figure}[h]
% \centering
% \begin{subfigure}{0.58\textwidth}
%   \centering
%   \noindent\fbox{%
%     \parbox{0.96\linewidth}{%
%     \vspace{-0.5em}
%       \begin{flushleft}\scriptsize{
%         \texttt{{\color{Gray}
% Human: {\color{magenta}move all the blocks into their matching bowls}.\\
% Scene: {\color{scene_description_color}There is a green block, a blue block, a yellow block, a green bowl, a blue bowl, a yellow bowl.}\\
% Robot: {\color{robot_action_color}Pick up the yellow block and place it in the yellow bowl.}\\
% Success Detector: {\color{success_detection_color}False.}\\
% Robot: {\color{robot_action_color}Pick up the yellow block and place it in the yellow bowl.}\\
% Robot: {\color{robot_action_color}Pick up the green block and place it in the green bowl.}\\
% Robot: {\color{robot_action_color}Pick up the blue block and place it in the blue bowl.}\\
% Success Detector: {\color{success_detection_color}False.}\\
% Robot: {\color{robot_action_color}Pick up the blue block and place it in the blue bowl.}\\
%         }
%       }}
%       \vspace{-0.5em}
%     \end{flushleft}
%   }}
%   % \caption{VLM + LM prompt.}
%   \label{fig:sub1}
% \end{subfigure}
% \begin{subfigure}{.195\textwidth}
%   \centering
%   \vspace{1.0em}
%   \includegraphics[width=1.0\linewidth]{figures/tabletop_env_scene}
%   % \caption{Example results on MS COCO images.}
%   \label{fig:sub3}
% \end{subfigure}
% \begin{subfigure}{.205\textwidth}
%   \centering
%   \vspace{1.0em}
%   \includegraphics[width=1.0\linewidth]{figures/tabletop_env_success}
%   % \caption{Example results on MS COCO images.}
%   \label{fig:sub2}
% \end{subfigure}

% \caption{\small \algname with a \textbf{{\color{scene_description_color}scene descriptor}} and a \textbf{{\color{success_detection_color}success detector}}, planning with GPT-3 to run language-conditioned \textbf{{\color{robot_action_color}robot policies}} (\eg via CLIPort \cite{shridhar2022cliport}) in a simulated environment with various objects on a table. It is able to respond to free-form human instructions (in \textbf{{\color{magenta}magenta}}).}
% \label{fig:tabletop_sim}
% \end{figure}
% \vspace{-1.0em}

% \subsection{Implementation Details}

% \subsubsection{Simulated Tabletop Rearrangement Environment}

% \subsubsection{Simulated Tabletop Rearrangement Environment}

==> Closed Loop LLM Planning CoRL 2022 2/extra/policies.tex <==
% \subsection{In Simulated Tabletop Rearrangement Environment}

% \subsection{In Real Tabletop Rearrangement Environment}

% The low-level policy for the real tabletop rearrangement environment is responsible for performing object-centric pick and place actions as instructed by the language model.
% The policy takes as input 1) the bounding boxes of all the objects in the scene, 2) the names of the object to pick and the target object for place, 3) the depth image corresponding to the RGB image from which object detection was done, 4) camera intrinsics, and 5) camera pose.
% It then outputs a 3D pick position and a 3D place location for the robot to follow.

% The pick position is the 3D coordinate of the center of the object bounding box in the robot base frame.
% This is obtained by first deprojecting the depth image pixel corresponding to the center of the pick object bounding box with the given camera intrinsics, then transforming this point from the camera frame to the robot frame with the given camera pose.
% Camera pose is known because it is a wrist camera, and we register the delta pose from the mounted camera to the robot end-effector.

% For the block stacking task, the place location is obtained the same way as the pick position.
% For the object sorting task, the place location is chosen to be a point in the target plate's bounding box that is farthest way from the bounding boxes of other objects.
% This is done to prevent undesired stacking behavior when placing objects into the plate, which may cause the object to roll off and fall off the table.

% To perform the pick and place motions, the robot moves to a position $15$cm above the intended pick or place position, and then it slowly lowers the end-effector until a $5$N contact force is detected.
% This is more robust than moving directly to the height obtained from the depth image due to depth sensor noises.
% We set a threshold for how low the end-effector can go for the object sorting task so picking inaccuracies do not result in accidentally picking up the plate.

% We add planar translation noise to the pick position by sampling the magnitude from a zero-mean Normal distribution and then sampling an angle from a uniform distribution on the unit circle.
% The standard deviation for the Normal distribution is $\sigma=1.5$cm for the block stacking task, $\sigma=0.7$cm for the object sorting task, and the samples are capped at $1.5\sigma$.

% \subsection{In Real Mobile Manipulator in a Kitchen Environment}

==> Closed Loop LLM Planning CoRL 2022 2/extra/success_detection.tex <==
% \subsection{In Simulated Tabletop Rearrangement Environment}

% \subsection{In Real Tabletop Rearrangement Environment}

% In the real tabletop rearrangement environment, success detection is done by comparing the 2D position of the center of the detected object bounding box after pick and place action with the intended 2D place position.
% By 2D we mean the x-y spatial coordinates in the base frame of the robot, not the image coordinates.
% These are obtained by deprojecting the detected bounding box centers from the depth image and converting the resulting 3D point from camera frame to base frame.
% The detector returns success if the difference between the two positions is less than a threshold.
% For the block stacking task, the threshold is $3$cm, and for the object sorting task it is $10$cm.
% While $3$cm is larger than half of the dimension of the blocks we use ($4$cm), it is more robust for our case because the center of the detected object bounding box is often not the center of the block.
% The threshold for object sorting is much higher, because for some objects, once they are placed in the plate, they may roll around until contact with the plate boundary.

% \subsection{In Real Mobile Manipulator in a Kitchen Environment}
% We trained a ``foresight" success detector on offline data collected from a combination of teleoperated demonstrations and autonomous roll-outs performing the low-level tasks. The input to the model consists of: (1) $o_0$, the initial image observation, (2) $o_f$, the final image observation after the policy chose to terminate its chosen skill execution, and (3) $l_k$, the low-level skill which the agent was trying to execute (\eg ``\texttt{\color{robot_action_color}{Pick coke can}}"). The model uses image encoders from CLIP \citep{radford2021learning} to embed $o_0$ and $o_f$, concatenate them, and fuse these representations with a fusion MLP. This image embedding is concatenated with the text embedding obtained by the CLIP text encoder, then passed through another MLP. The output of the model is a scalar denoting the probability of the agent succeeding at the specified task (Figure \ref{fig:saycan_sd_fs}). The model is trained with the binary cross entropy loss with respect to the ground truth binary label. We fine tune the CLIP model as well during the training. At inference time when using with the robot, we output the text \texttt{\color{success_detection_color}{[Success: no]}} when the probability is below a certain threshold. 

% To reduce false positive predictions, we trained a separate ``hindsight" success predictor model. Given the first and last observation, the model outputs a probability distribution over all the possible skills. We used this model to disambiguate between possible tasks that the agent may have achieved. To train this model, we use the symmetric contrastive loss as used in CLIP (Figure \ref{fig:saycan_sd_hs}). At inference time, similar to the CLIP model, we take a dot product between the image-fusion embedding and the text embeddings and apply softmax with a learned temperature.

% We combine the foresight and hindsight model by first thresholding the probability from the foresight model by some value $\tau$. If the probability is above, then we run the hindsight model and only predict success if the argmax across all skills is indeed the foresight task.

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%     \includesvg[width=\linewidth]{figures/SayCan_SD.svg}
%     \caption{Foresight success detector}
%     \label{fig:saycan_sd_fs}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.48\textwidth}
%     \includesvg[width=\linewidth]{figures/SayCan_SD_Hindsight.svg}
%     \caption{Hindsight success detector}
%     \label{fig:saycan_sd_hs}
%     \end{subfigure}
%     \caption{Success Detection architecture used for the Kitchen Environment. (\textit{Left}) The foresight model predicts whether a given instruction was successfully achieved between the first and last image. (\textit{Right}) The hindsight model fine-tuned via contrastive loss as used in CLIP \citep{radford2021learning}. At inference time, the model is used infer among the possible instructions which one was achieved.}
%     \label{fig:saycan_sd}
% \end{figure}

==> Closed Loop LLM Planning CoRL 2022 2/introduction-arxiv.tex <==

Intelligent and flexible embodied interaction requires robots to be able to deploy large repertoires of basic behaviors in appropriate ways, sequence these behaviors as needed for long horizon tasks, and also recognize when to switch to a different approach if a particular behavior or plan is unsuccessful.
High-level planning, perceptual feedback, and low-level control are just a few of the sub-tasks that would need to be seamlessly combined together to perform the sort of reasoning required for an embodied agent, such as a robot, to intelligently act in the world.
While conventionally these challenges have been approached from the perspective of planning (e.g., TAMP~\citep{kaelbling2013integrated}) or hierarchical learning (e.g., HRL~\citep{barto2003recent}), effective high-level reasoning about complex tasks also requires semantic knowledge and understanding of the world.

One of the remarkable observations in recent machine learning research is that large language models (LLMs) can not only generate fluent textual descriptions, but also appear to have rich internalized knowledge about the world~\citep{petroni2019language,jiang2020can,davison2019commonsense,talmor2020olmpics,roberts2020much}. When appropriately conditioned (e.g., prompted), they can even carry out some degree of deduction and respond to questions that appear to require reasoning and inference~\citep{chowdhery2022palm,brown2020language,wei2022chain,kojima2022large,lampinen2022can,nye2021show}.
This raises an intriguing possibility: beyond their ability to interpret natural language instructions,
can language models further serve as reasoning models that combine multiple sources of feedback and become interactive problem solvers for embodied tasks, such as robotic manipulation?


Prior studies show that language helps humans internalize our knowledge and perform complex relational reasoning through \textit{thinking in language}~\citep{vygotsky2012thought,carruthers1998thinking,vygotsky1994tool,vygotsky1967play,colas2022vygotskian}. Imagine the ``inner monologue'' that happens when a person tries to solve some task: ``I have to unlock the door; let me try to pick up the key and put it in the lock... no, wait, it doesn't fit, I'll try another one... that one worked, now I can turn the key.''
The thought process in this case involves choices about the best immediate action to solve the high-level task (``pick up the key''), observations about the outcomes of attempted actions (``it doesn't fit''), and corrective actions that are taken in response to these observations (``I'll try another one'').
Inspired by the human thought process, we propose that such an inner monologue is a natural framework for incorporating feedback for LLMs.


Our work studies these questions by combining LLMs with various sources of textual feedback, only utilizing few-shot prompting without any additional training. 
We observe that similarly to recent work~\citep{zeng2022socratic}, natural language provides a universal and interpretable interface for such grounding of model communication and allows them to incorporate their conclusions in an overarching inner monologue driven by a language model.
While prior work has investigated using language models as planners \cite{huang2022language,ahn2022can} or incorporating multimodal-informed perception through language \cite{zeng2022socratic}, to the best of our knowledge no work has studied the critical link of not only planning with language, but also informing \textit{embodied feedback with language}, which we investigate in this work.


Specifically, we study methods and sources of feedback for closing the agent-environment loop via an inner monologue and their impact on downstream execution success and new capabilities arising from such interaction.
In particular, we combine multiple perception models that perform various tasks such as language-conditioned semantic classification or language-based scene description, together with feedback provided by a human user that the robot is cooperating with.
To execute the commands given by a user, the actions are chosen from a set of pre-trained robotic manipulation skills together with their textual descriptions that can be invoked by a language model.
Our proposed system~\algname chains together these various components (perception models, robotic skills, and human feedback) in a shared language prompt, enabling it to successfully perform user instructions.

%\todo{describe the results and contributions}
Finally, we show that~\algname, without requiring additional training beyond a frozen language model and pre-trained robotic skills, can accomplish complex, long-horizon, and unseen tasks in simulation as well as on two real-world robotic platforms. Notably, we show that it can efficiently retry under observed stochastic failure, replan under systematic infeasibility, or request human feedback for ambiguous queries, resulting in significantly improved performance in dynamical environments. As a demonstration of the versatility of LLMs and grounded closed-loop feedback, we additionally show several surprising capabilities emerging from the inner monologue formulation, including continued adaptation to new instructions, self-proposed goals, interactive scene understanding, multilingual interactions, and more.


==> Closed Loop LLM Planning CoRL 2022 2/related.tex <==
\paragraph{Task and Motion Planning.}
% \textit{(General prior task planning works)}
Task and motion planning \cite{kaelbling2010hierarchical,srivastava2014combined} requires simultaneously solving a high-level, discrete task planning problem \cite{fikes1971strips,sacerdoti1975structure,nau1999shop}, and a low-level, continuous motion planning problem \cite{lavalle2006planning}. 
Traditionally, this problem has been solved through optimization \citep{toussaint2015logic,toussaint2018differentiable} or symbolic reasoning \citep{fikes1971strips,nau1999shop}, but more recently machine learning has been applied to aspects of the problem via learned representations, learned task-primitives, and more~\citep{Eysenbach2019search,xu2018neural,xu2019regression,silver2022inventing,shah2022value,srinivas2018universal,kurutach2018learning,akakzia2021grounding,pirk2020modeling}.
Some works utilize language for planning and grounding~\citep{kollar2010toward,tellex2011understanding,bollini2013interpreting,tellex2014asking,kollar2014grounding,blukis2019learning}.
Others have approached the problem through hierarchical learning~\citep{Nair2020HierarchicalFS,xia2021relmogen,shah2022value,li2020hrl4in,Jiang2019LanguageAA,hafner2022deep, mirchandani2021ella}.
In this work, we leverage pre-trained LLMs and their semantic knowledge, along with trained low-level skills, to find feasible plans.

% \HC{Some works on HRL with language: \citep{jiang2019language,mirchandani2021ella}, manipulation \citep{akakzia2021grounding} discovers abstract goals related to language instructions using intrinsically motivated RL.}  % tompson: Incorporated these.

\paragraph{Task Planning with Language Models.}
Various prior works have explored using language as a space for planning~\citep{jansen2020visually,sharma2021skill,huang2022language,li2022pre,ahn2022can,zeng2022socratic}. Similar to ours are recent task planning approaches that leverage pre-trained autoregressive LLMs to decompose abstract, high-level instructions into a sequence of low-level steps executable by an agent~\citep{huang2022language,ahn2022can} in a zero-shot manner. Specifically,~\citet{huang2022language} prompt GPT-3~\citep{brown2020language} and Codex~\citep{chen2021evaluating} to generate action plans for embodied agents, where each action step is semantically translated to an admissible action with a Sentence-RoBERTa model~\citep{liu2019roberta,reimers2019sentence}. 
% TODO: comment on the autoregressive generation aspect too?
\mbox{SayCan}~\citep{ahn2022can} instead grounds the actions by multiplying each candidate action's probability under FLAN~\citep{wei2021finetuned} with the action's value function, which serves as a proxy for affordance~\citep{shah2022value}. However, both approaches effectively produce the plan while assuming that each proposed step is executed successfully by the agent. As a result, these approaches may not be robust in handling intermediate failures in dynamic environments or with poor lower level policies. We explore in~\algname ways to incorporate grounded feedback from the environment into the LLM as we produce each step in the plan. 

\paragraph{Fusing Vision, Language, and Control in Robotics.}
% Be specific that this is large models on semi-supervised objectives.
%\paragraph{End-to-end Visual Language and Control Models in Robotics.}
Various works have investigated strategies for the challenging problem of fusing vision, language, and control~\citep{paxton2019prospection,stepputtis2020language,blukis2020few,lynch2021language,chen2021joint,mees2022matters,yan2022intra}.
% \citet{lynch2021language} introduced a method to train vision-and-language-conditioned imitation learning on  unstructured robotic experience, and conditionable on free-form language, enabled in part by the use of pretrained LLMs to encode input text. %This work demonstrated some live collaboration where a user can adjust instructions to help the robot achieve tasks (for example ``move back" to get unstuck), albeit as a one-sided conversation.
While pretrained LLMs typically train only on text data, pretrained visual-language models (e.g., CLIP \citep{radford2021learning}) are trained on joint image(s) and corresponding text captions via variants of masked language modeling (MLM) objective \citep{devlin2018bert,lu2019vilbert,wang2021simvlm,suglia2021embodied}, contrastive loss \citep{chen2020big,jain2021mural,radford2021learning} or other supervised objectives\citep{sun2022plate,sener2019zero}. 
%CLIP \citep{radford2021learning} uses contrastive learning to align vision and language representation from millions of image-text pairs from the internet.
CLIP has been employed in several robotics and embodied settings in zero-shot manner \citep{khandelwal2022simple}, or combined with Transporter networks \citep{zeng2020transporter} as in CLIPort \citep{shridhar2022cliport}.
Socratic Models \citep{zeng2022socratic} combines several foundation models (e.g., GPT-3 \citep{brown2020language}, ViLD \citep{gu2021vild}) and language-conditioned policies, using language as the common interface, and demonstrated manipulating objects in a simulated vision-based robotic manipulation environment.
% ~\citet{yan2022intra} also explore using language as an abstraction to form ``intra-agent speech'' for embodied tasks, where an image captioning model is trained using human-labeled captions to facilitate down-stream behavioral learning. In contrast,~\algname leverages \textit{existing} knowledge in frozen LLMs to solve temporally-extended tasks in dynamic environments, by chaining together pre-trained skills and embodied feedback from learned models.

% Others to add:
% \begin{itemize}
    % \item MAC - \citep{yu2022modular} - maybe?
    % \item PlaTe - \citep{sun2022plate} - definite add
    % \item Zero-shot anticipation for instructional activities \citep{sener2019zero} - language model to break down tasks for instruction following.
% \end{itemize}

% \begin{itemize}
%     \item LLMs as planners (Wenlong's, SayCan). Limited to open loop planning from LLMs.
%     \item VLMs, CLIPort
%     \item Socratic models
% \end{itemize}

==> extra/implementation_details.tex <==
% \subsection{Figures Moved to Appendix from Main Text}

% % This was moved from main text to save space.
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=1.0\textwidth]{figures/flowchart_decision_making}
%   \caption{\small\textbf{\algname Reacts to Feedback} The planner is able to react to textual feedback from success detector, object detection and human preference. After each environment feedback, the planner updates its predictions in language space for the next action.}
%   \todo{caption}
%   \label{fig:saycan-flow-chart}
% \end{figure}

% \begin{figure}[h]
% \centering
% \begin{subfigure}{0.58\textwidth}
%   \centering
%   \noindent\fbox{%
%     \parbox{0.96\linewidth}{%
%     \vspace{-0.5em}
%       \begin{flushleft}\scriptsize{
%         \texttt{{\color{Gray}
% Human: {\color{magenta}move all the blocks into their matching bowls}.\\
% Scene: {\color{scene_description_color}There is a green block, a blue block, a yellow block, a green bowl, a blue bowl, a yellow bowl.}\\
% Robot: {\color{robot_action_color}Pick up the yellow block and place it in the yellow bowl.}\\
% Success Detector: {\color{success_detection_color}False.}\\
% Robot: {\color{robot_action_color}Pick up the yellow block and place it in the yellow bowl.}\\
% Robot: {\color{robot_action_color}Pick up the green block and place it in the green bowl.}\\
% Robot: {\color{robot_action_color}Pick up the blue block and place it in the blue bowl.}\\
% Success Detector: {\color{success_detection_color}False.}\\
% Robot: {\color{robot_action_color}Pick up the blue block and place it in the blue bowl.}\\
%         }
%       }}
%       \vspace{-0.5em}
%     \end{flushleft}
%   }}
%   % \caption{VLM + LM prompt.}
%   \label{fig:sub1}
% \end{subfigure}
% \begin{subfigure}{.195\textwidth}
%   \centering
%   \vspace{1.0em}
%   \includegraphics[width=1.0\linewidth]{figures/tabletop_env_scene}
%   % \caption{Example results on MS COCO images.}
%   \label{fig:sub3}
% \end{subfigure}
% \begin{subfigure}{.205\textwidth}
%   \centering
%   \vspace{1.0em}
%   \includegraphics[width=1.0\linewidth]{figures/tabletop_env_success}
%   % \caption{Example results on MS COCO images.}
%   \label{fig:sub2}
% \end{subfigure}

% \caption{\small \algname with a \textbf{{\color{scene_description_color}scene descriptor}} and a \textbf{{\color{success_detection_color}success detector}}, planning with GPT-3 to run language-conditioned \textbf{{\color{robot_action_color}robot policies}} (\eg via CLIPort \cite{shridhar2022cliport}) in a simulated environment with various objects on a table. It is able to respond to free-form human instructions (in \textbf{{\color{magenta}magenta}}).}
% \label{fig:tabletop_sim}
% \end{figure}
% \vspace{-1.0em}

% \subsection{Implementation Details}

% \subsubsection{Simulated Tabletop Rearrangement Environment}

% \subsubsection{Simulated Tabletop Rearrangement Environment}

==> extra/policies.tex <==
% \subsection{In Simulated Tabletop Rearrangement Environment}

% \subsection{In Real Tabletop Rearrangement Environment}

% The low-level policy for the real tabletop rearrangement environment is responsible for performing object-centric pick and place actions as instructed by the language model.
% The policy takes as input 1) the bounding boxes of all the objects in the scene, 2) the names of the object to pick and the target object for place, 3) the depth image corresponding to the RGB image from which object detection was done, 4) camera intrinsics, and 5) camera pose.
% It then outputs a 3D pick position and a 3D place location for the robot to follow.

% The pick position is the 3D coordinate of the center of the object bounding box in the robot base frame.
% This is obtained by first deprojecting the depth image pixel corresponding to the center of the pick object bounding box with the given camera intrinsics, then transforming this point from the camera frame to the robot frame with the given camera pose.
% Camera pose is known because it is a wrist camera, and we register the delta pose from the mounted camera to the robot end-effector.

% For the block stacking task, the place location is obtained the same way as the pick position.
% For the object sorting task, the place location is chosen to be a point in the target plate's bounding box that is farthest way from the bounding boxes of other objects.
% This is done to prevent undesired stacking behavior when placing objects into the plate, which may cause the object to roll off and fall off the table.

% To perform the pick and place motions, the robot moves to a position $15$cm above the intended pick or place position, and then it slowly lowers the end-effector until a $5$N contact force is detected.
% This is more robust than moving directly to the height obtained from the depth image due to depth sensor noises.
% We set a threshold for how low the end-effector can go for the object sorting task so picking inaccuracies do not result in accidentally picking up the plate.

% We add planar translation noise to the pick position by sampling the magnitude from a zero-mean Normal distribution and then sampling an angle from a uniform distribution on the unit circle.
% The standard deviation for the Normal distribution is $\sigma=1.5$cm for the block stacking task, $\sigma=0.7$cm for the object sorting task, and the samples are capped at $1.5\sigma$.

% \subsection{In Real Mobile Manipulator in a Kitchen Environment}

==> extra/success_detection.tex <==
% \subsection{In Simulated Tabletop Rearrangement Environment}

% \subsection{In Real Tabletop Rearrangement Environment}

% In the real tabletop rearrangement environment, success detection is done by comparing the 2D position of the center of the detected object bounding box after pick and place action with the intended 2D place position.
% By 2D we mean the x-y spatial coordinates in the base frame of the robot, not the image coordinates.
% These are obtained by deprojecting the detected bounding box centers from the depth image and converting the resulting 3D point from camera frame to base frame.
% The detector returns success if the difference between the two positions is less than a threshold.
% For the block stacking task, the threshold is $3$cm, and for the object sorting task it is $10$cm.
% While $3$cm is larger than half of the dimension of the blocks we use ($4$cm), it is more robust for our case because the center of the detected object bounding box is often not the center of the block.
% The threshold for object sorting is much higher, because for some objects, once they are placed in the plate, they may roll around until contact with the plate boundary.

% \subsection{In Real Mobile Manipulator in a Kitchen Environment}
% We trained a ``foresight" success detector on offline data collected from a combination of teleoperated demonstrations and autonomous roll-outs performing the low-level tasks. The input to the model consists of: (1) $o_0$, the initial image observation, (2) $o_f$, the final image observation after the policy chose to terminate its chosen skill execution, and (3) $l_k$, the low-level skill which the agent was trying to execute (\eg ``\texttt{\color{robot_action_color}{Pick coke can}}"). The model uses image encoders from CLIP \citep{radford2021learning} to embed $o_0$ and $o_f$, concatenate them, and fuse these representations with a fusion MLP. This image embedding is concatenated with the text embedding obtained by the CLIP text encoder, then passed through another MLP. The output of the model is a scalar denoting the probability of the agent succeeding at the specified task (Figure \ref{fig:saycan_sd_fs}). The model is trained with the binary cross entropy loss with respect to the ground truth binary label. We fine tune the CLIP model as well during the training. At inference time when using with the robot, we output the text \texttt{\color{success_detection_color}{[Success: no]}} when the probability is below a certain threshold. 

% To reduce false positive predictions, we trained a separate ``hindsight" success predictor model. Given the first and last observation, the model outputs a probability distribution over all the possible skills. We used this model to disambiguate between possible tasks that the agent may have achieved. To train this model, we use the symmetric contrastive loss as used in CLIP (Figure \ref{fig:saycan_sd_hs}). At inference time, similar to the CLIP model, we take a dot product between the image-fusion embedding and the text embeddings and apply softmax with a learned temperature.

% We combine the foresight and hindsight model by first thresholding the probability from the foresight model by some value $\tau$. If the probability is above, then we run the hindsight model and only predict success if the argmax across all skills is indeed the foresight task.

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%     \includesvg[width=\linewidth]{figures/SayCan_SD.svg}
%     \caption{Foresight success detector}
%     \label{fig:saycan_sd_fs}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.48\textwidth}
%     \includesvg[width=\linewidth]{figures/SayCan_SD_Hindsight.svg}
%     \caption{Hindsight success detector}
%     \label{fig:saycan_sd_hs}
%     \end{subfigure}
%     \caption{Success Detection architecture used for the Kitchen Environment. (\textit{Left}) The foresight model predicts whether a given instruction was successfully achieved between the first and last image. (\textit{Right}) The hindsight model fine-tuned via contrastive loss as used in CLIP \citep{radford2021learning}. At inference time, the model is used infer among the possible instructions which one was achieved.}
%     \label{fig:saycan_sd}
% \end{figure}
